Touchtone leakage attacks via smartphone sensors: mitigation without hardware modification

Smartphone motion sensors provide a concealed mechanism for eavesdropping on acoustic information, like touchtones, emitted by a device. Eavesdropping on touchtones exposes credit card information, banking pins, and social security card numbers to malicious 3rd party apps requiring only motion sensor data. This paper's primary contribution is an analysis rooted in physics and signal processing theory of several eavesdropping mitigations, which could be implemented in a smartphone update. We verify our analysis imperially to show how previously suggested mitigations, i.e. a low-pass filter, can undesirably reduce the motion sensor data to all applications by 83% but only reduce an advanced adversary's accuracy by less than one percent. Other designs, i.e. anti-aliasing filters, can fully preserve the motion sensor data to support benign application functionality while reducing attack accuracy by 50.1%. We intend for this analysis to motivate the need for deployable mitigations against acoustic leakage on smartphone motion sensors, including but not limited to touchtones, while also providing a basis for future mitigations to improve upon.

==> tabs/impact.tex <==
\begin{table}[!t]
    \centering
    \begin{tabular}{p{0.95cm} || p{.6cm} | p{.6cm}  | p{.6cm} || p{1.5cm}  | p{1.5cm} }
        \multirow{3}{.95cm}{Single Digit Accuracy} & \multicolumn{3}{c||}{Bank Pin Recognition \%} & \multicolumn{2}{c}{Credit Card ID Recognition \%} \\ \cline{2-6}
        & \multirow{2}{.75cm}{4 digit} & \multirow{2}{.75cm}{5 digit} & \multirow{2}{.75cm}{6 digit} & 16~digit~card & 18~digit~card \\
        & & & & {\textbackslash}w~9~digit~ID & {\textbackslash}w~11~digit~ID \\ \hline
        \textbf{75\%} &	32\% &	24\% &	18\% &	8\% &	4\% \\ \hline
        80\% &	41\% &	33\% &	26\% &	13\% &	9\% \\ \hline
        85\% &	52\% &	44\% &	38\% &	23\% &	17\% \\ \hline
        90\% &  66\% &  59\% &	53\% &	39\% &	31\% \\ \hline
        95\% &	81\% &  77\% & 	74\% &  63\% &	57\%
    \end{tabular}
    \caption{Calculations for first guess accuracy of a bank pin or credit card identification number given the single digit recognition accuracy. In prior tests, \implementation achieved roughly 75\% (in bold) on two of the four tested phones.\con{redo for new accuracies.}}
    \label{tab:impact}
\end{table}

==> tabs/parameter-search.tex <==
\begin{table}[!t]
    \centering
    \begin{tabular}{p{2cm} | p{2cm} | p{3cm}}
        & \textbf{XGBoost} & Random Forest \\ \hline
        \textbf{Time/Freq} & \textbf{74.1}\% & 73.2\% \\
        MFCCs & 70.1\% & 67.0\% \\
        
        \end{tabular}
    \caption{Highest results for a randomized grid searches for features and classifiers using isolated word recognition data collected on a Pixel~2 in a conference room.. }
    \label{tab:parameter-search}
\end{table}

==> tabs/setup-info.tex <==

\begin{table}[!t]
% \fontsize{10}{7.2}\selectfont
    \centering
    \begin{tabular}{l | l | l | l}
        Location & Noise Level & Speaker Setup & Devices \\ \hline
        Conference Room & 53 dB~SPL & Internal Phone Speaker & Pixel~1, Pixel~2, Galaxy~S8, Galaxy~S9 \\
        Server Room & 67 dB~SPL & Internal Phone Speaker & Pixel~1, Pixel~2, Galaxy~S8, Galaxy~S9 \\
        Acoustic Chamber & 31 dB~SPL & External Speaker & LSM9DS1 Breakout, ADXL337 Breakout
    \end{tabular}
    \caption{Different data collection setups. Phones were placed in more realistic conditions while the breakout boards were placed in an acoustic isolation chamber to eliminate outside variables. The phones produced their own sound, while the breakout boards were placed 30 to 40cm away from an external speaker placed on the same table.}
    \label{tab:setup_info}
\end{table}
